Spatial Interpolants

We propose Splinter, a new technique for proving properties of heap-manipulating programs that marries (1) a new separation logic-based analysis for heap reasoning with (2) an interpolation-based technique for refining heap-shape invariants with data invariants. Splinter is property directed, precise, and produces counterexample traces when a property does not hold. Using the novel notion of spatial interpolants modulo theories, Splinter can infer complex invariants over general recursive predicates, e.g., of the form all elements in a linked list are even or a binary tree is sorted. Furthermore, we treat interpolation as a black box, which gives us the freedom to encode data manipulation in any suitable theory for a given program (e.g., bit vectors, arrays, or linear arithmetic), so that our technique immediately benefits from any future advances in SMT solving and interpolation.

==> Makefile <==
.PHONY: preview
preview:
	latexmk -pvc -jobname=paper -f "\def\preview{}\input{paper}"

.PHONY: paper.pdf
paper.pdf:
	latexmk -g paper

dist:
	mkdir berdine
	mkdir berdine/figs
	cp paper.tex preamble.tex intro2.tex example.tex prelims.tex spint.tex snint.tex bounded_abduction.tex eval.tex related.tex paper.bib llncs.cls splncs03.bst mathpartir.sty copyright-lncs-signed.pdf paper.pdf paper.bbl berdine
	cp figs/arch.pdf figs/ex.pdf berdine/figs
	tar czf berdine.tgz berdine


==> conc.tex <==
\section{Discussion}
We have presented \alg,
a new technique for proving safety
properties of programs requiring heap
and data reasoning.
\alg combines a new path-based separation logic
analysis with first-order interpolation techniques
for inferring intricate invariants.
%
By bringing the advantages of the path-based refinement approach that has
proven to be extremely effective in the domain of numerical and
control-sensitive property verification to the domain of combined heap and
data verification, we believe \alg is an important step in creating precise
and generic automatic heap/data analyses.

In this work we compute spatial($\mathcal{T}$) interpolants
in a two-tiered manner: computing spatial interpolants followed
by theory interpolants. This suffers from the problem
that the computed spatial interpolants might not have theory interpolants
(even though refinable spatial interpolants may exist),
in which case our algorithm reverts to the strongest spatial interpolants.
In the future, we would like to study
systematically searching the space of spatial interpolants,
until a set of spatial interpolants that can be refined with theory
interpolants is found.
We believe this can be performed in a counterexample-guided manner,
where an unsolvable set of Horn clauses can inform us how to 
modify our spatial interpolants.


%There are several directions in which our work can be extended,
%such as handling arbitary recurisve shape predicates and
%existential properties of lists.
%%Additionally, two interesting, important, and non-trivial open problems arise from our proposed
%technique:
%\begin{compactitem}
%\item Finding a weak (ideally, \emph{maximally} weak) \logic formula
%that under-approximates a logical conjunction of two \logic formulas.
%Applications of this operation transcend our proposed technique.
%For example, this may be useful for 
%combining invariants produced by different shape analysis tools.
%\item Systematically searching the space of spatial interpolants,
%until a set of spatial interpolants which can be refined with theory
%interpolants is found.
%We believe this can be performed using a counterexample-guided manner,
%where an unsolvable set of Horn clauses can inform us how to 
%modify our spatial interpolants.
%\end{compactitem}
%We plan to study these problems in future work.
%
%% In the future, we plan on extending our
%% technique to ,
%% in order to allow verification of complex programs.
%% Additionally, we are also interested in extending \alg
%% to reason about 



%% In our experimental evaluation, our heuristic
%% solutions to these two problems have been sufficient
%% for handling our benchmarks.


==> conj.tex <==
\section{Putting it All Together} \label{sec:alg}
\begin{itemize}
\item Describe how from path interpolants we can go to full proofs -- impact style.
\item Describe how we need to take prefixes of paths in cases where the whole path
does not have a proof of correctness.
\item Finally, maybe describe how we can perform conjunction -- or we can handwave it
if it's too much work.
\end{itemize}


==> intro.tex <==
\section{Introduction} \label{sec:intro}
The past decade has witnessed
significant advances in the % never-ending
quest for efficient automated software verification techniques.
For example, 
advances such as 
predicate abstraction~\cite{Graf97,Ball01,Henzinger2002},
interpolation~\cite{McMillan2006},
and SMT solving~\cite{Barrett09}
have facilitated efficient verification of 
control-sensitive and numerical properties.
Within the same arena of numerical properties, techniques employing
numerical abstract domains~\cite{Cousot77} have been successfully
applied to large safety-critical systems~\cite{Blanchet03}.
On the other hand, in the heap world, scalable techniques
based on separation logic~\cite{Reynolds2002} have been
applied to proving memory safety of % very
large
low-level software~\cite{Calcagno09}.
%
However, combined heap and data reasoning is comparatively under-explored.
For instance, memory safety analyses generally either try to prove array
accesses are within bounds assuming pointers to arrays are valid, or to prove
accesses through pointers are valid assuming accesses to valid arrays are
within bounds.

This paper is concerned with verifying
safety properties that require heap as well as
data reasoning.
Consider, for example, a program
that stores array indices in a linked list and then
uses them to access the array,
% such scenarios are prevalent in low-level software.
% Another important class of programs where heap and data
% reasoning is required is programs that manage
%memory with \emph{reference counting}.
or a program that uses reference counting to manage memory.
In order to prove memory safety of such programs, we need
%% to track arithmetic and heap invariants.
to be able to infer intricate invariants that involve
both data and heap shape.
%% To prove safety of array accesses in the said program, 
%% one has to infer the intricate invariant 
%% that all elements of the linked
%% list lie within the bounds of the accessed array.
The aforementioned techniques are unable %will not be able
to prove safety of such programs:
software model checking techniques
track only very shallow heap information (e.g., using traditional pointer analysis),
and most separation logic and shape analysis techniques
do not track data invariants of heap data structures.

In this paper, we propose \alg, a novel safety verification
algorithm that is able to prove properties
requiring integrated heap and data reasoning.
\alg marries (1) a new form of rich separation logic
reasoning, for \emph{lazily} inferring heap invariants,
with (2) interpolation-based reasoning, for strengthening
heap invariants with \emph{data refinements}.
%We describe our technique and summarize its novel features as follows:
\begin{figure}[t]
\centering
\includegraphics[scale=0.32]{figs/arch.pdf}
\caption{Overview of \alg verification algorithm.}
\label{fig:arch}
\end{figure}



%\paragraph{Path Sampling}
Given a program $P$ and safety property $\varphi$,
\alg constructs a proof that $P$ is memory safe and satisfies $\varphi$
by \emph{sampling paths} through the control-flow graph of $P$
and proving them safe.
That is, by proving safety of a finite number
of paths (samples), we construct a proof of the whole program.
This is inspired by McMillan's \emph{lazy abstraction with interpolants} (\impact)
verification technique~\cite{McMillan2006},
where \emph{Craig interpolants} are used to prove
% correctness of
individual paths.
%% Adopting a \emph{path sampling} verification strategy makes
%% our algorithm:
The \emph{path sampling} methodology (e.g., as in~\cite{McMillan2006,Beyer07,Heizmann10})
enables the following features:
\vspace{-.05in}
\begin{enumerate}
%% \item \emph{Path-sensitive}:  This allows us to avoid 
%% imprecision due to lossy join operations often employed
%% by abstract domains.
%% \zak{Is this terminology standard in model checking lit?  I think
%%   path-sensitivity is one of those things that means different things in
%%   different communities.  Path-based?  I'm also a little confused about the
%%   groupings here.  For example, I don't see the connection between
%%   counter-examples and property direction.  Maybe we should use ``refinement-based''?}
%% %
%% \jjb{Yes, I don't think path sampling has nothing to do with path
%%   sensitivity.  Many of the shape analyses are path sensitive
%%   (powerset domains) and don't use approximate joins.  The real
%%   significance, to my understanding, of the path sampling aspect is
%%   that it enables the underapproximation of weakest preconditions, as
%%   well as the refinement of spatial with theory information, to be
%%   done with respect to \emph{symbolic} instead of \emph{abstract}
%%   traces.  The symbolic traces are both precise and feasible, so
%%   refinement can add any information true in the symbolic rather than
%%   only that which happened to survive through a backward transformer
%%   (along a possibly infeasible path).  Also, since the spatial
%%   interpolant formulas are bounded between the symbolic and weakest
%%   pre of true, at each step as much information can be abstracted away
%%   as possible, without needing to fix a single abstraction function
%%   for the entire path, let alone program.  There is an aspect
%%   analogous to lazy abstraction here.  But ``refinement-based'' seems
%%   too underspecified to me.}
%% %
%% \aws{Yeah, most shape domains are powerset domains, but I intended this to be a point
%% on numerical domains used. I wasn't happy about the groupings too when I wrote it, but since no
%% one complained I didn't change it, but here we are...What do you suggest we say here?
%% I can try to rewrite it.}
\item \emph{Path-based refinement}: %This allows us to avoid
  This supports a progress guarantee by tightly correlating program
  exploration with refinement, and by avoiding imprecision due to
  lossy join and widening operations employed by abstract domains.  \alg does
  not report false positives, and produces counterexamples for violated
  properties.
  This comes, as usual, at the price of potential divergence.
%\jjb{Should we admit: This comes, as usual, at the price of potential divergence.}
%\zak{I think so.}
\item \emph{Property-direction}: Rather than seeking the strongest
  invariant possible, we compute one that is \emph{just strong enough} to
  prove that a desired property holds.  Property direction enables scalable
  reasoning in rich program logics (like the one described in this paper),
  which is necessary for proving properties combining data and the heap.

%% The idea of property-directed verification is to compute an invariant that is,
%% rather than the strongest possible, \emph{just strong enough} to prove that
%% some desired property holds \cite{Henzinger2002,McMillan2006}.  The key
%% benefit of property direction is that it enables scalable reasoning in rich
%% program logics (as described below). 
%% Moreover, our algorithm does not suffer from precision
%% loss due to widening, and produces feasible
%% counterexample traces in case a property is not satisfied.
%% Of course, as with other property-directed techniques, 
%% this comes at the expense of possible non-termination.
\end{enumerate}

Figure~\ref{fig:arch} summarizes the high-level
operation of our algorithm.
Notice that, at one extreme, given a program with no heap manipulation,
\alg only computes theory interpolants
and behaves exactly like
%McMillan's \impact algorithm.
\impact.
One can thus view \alg as a proper
extension of \impact to heap manipulating programs.
At the other extreme, given
a program with no data manipulation, our algorithm is a new shape analysis
that uses path-based relaxation to construct memory safety proofs in
separation logic.
%At the other extreme, given a program with no data manipulation,
%our algorithm is a new property-directed 
%% \jjb{There is something odd about calling this ``property-directed'' when there is no data, since the property, memory safety, is the same for all paths of all programs.  But, on the other hand, abstracting the assertions on a path as much as possible while still proving memory safety is quite different from using a fixed abstraction.  I'm not sure that readers will fully appreciate this aspect.}
%% \zak{I agree this sounds a little weird.  Maybe: ``At the other extreme, given
%%   a program with no data manipulation, our algorithm is a new shape analysis
%%   which uses path-based refinement to construct memory safety proofs in
%%   separation logic.''}
%% \jjb{Better, but at this extreme, is there really any ``refinement''.  Perhaps ``path-based relaxation''?  I think that the key point that is likely to go unappreciated is how the path-based approach allows weakening the proofs beyond what one could get away with using a fixed abstraction.  Not sure how to say it so that readers without an intuitive grasp of interpolation-based SMC appreciate it.}
%% \zak{Fair enough -- I'm good with ``path-based relaxation''}
%separation logic--based shape analysis.
Thus, \alg is a step forward in the direction towards fully automatic
 verification: since it integrates both numerical and heap reasoning,
it obviates the need to choose which category of verification tool to
apply to a program of interest.  Moreover, it can be used to prove properties
that lie beyond the scope of either category.

There is some prior work on combined heap and data analysis, discussed in
Section~\ref{sec:rel}, but none enjoys
\alg's two key features: path-based refinement and property-direction.
% the two key features of \alg described above.


%% Thus, one of the advantages of \alg is its generality
%% and flexibility. Given some program and a safety property,
%% it is often non-trivial to tell if proving the property
%% requires heap reasoning, numerical data reasoning, or both.
%% \alg simplifies the job of choosing an appropriate verification tool
%% by integrating both kinds of reasoning.

At the core of \alg is the idea of \emph{spatial interpolants modulo theories},
which are used to construct a proof of correctness of a given program path.% ;
% we describe them below


\paragraph{Spatial Interpolants}
To prove a program path $\pi$ safe,
we first construct a Hoare-style proof of 
memory safety of $\pi$
% this really should be an en dash, since it is (separation logic)-based not separation (logic-based)
using a new separation logic--based technique.
We call the annotations along the path \emph{spatial path interpolants},
since, in the style of interpolation-based verification,
% they are \emph{in between}
their logical strength is \emph{in between} that of
the sequences of strongest postconditions and of weakest preconditions.
Effectively, spatial interpolants tell us 
which parts of the heap, and their structure, we should remember at each point
along the path in order to ensure safe execution thereafter.
Consequently, our technique does not suffer
from the imprecision incurred by forward-running %based separation logic 
shape analyses, which might
\emph{abstract too much} (e.g., by widening) and report unsafe memory operations
in a safe program. 

Our spatial interpolation procedure is a two step process that first
symbolically executes the path in a forward pass and then derives a weaker
proof using a backward pass.  The backward pass can be thought of as an
under-approximate weakest precondition computation, which uses the symbolic
heap from the forward pass to guide the under-approximation.
%
This second pass is the principal point at which heuristic approximation is
involved.  The approximation strives toward the weakest preconditions while, in
the limit, ``unsuccessful'' approximation yields the overly-strong proof from
the first pass.

%% To enable path-based reasoning and achieve
%% this precision, we propose computing spatial interpolants for a path
%% using a \emph{bounded} form of \emph{abductive inference},
%% where for each program location on the path we ask the 
%% question: \emph{what do we need to know
%% about the heap at this point to ensure memory safe execution?}
%% That is, we look for a weakening of the set of reachable
%% heap configurations (states) at a given location
%% that is sufficient to ensure memory safe execution.

\paragraph{Spatial Interpolants Modulo Theories}
Given a memory safety proof of a path $\pi$ (spatial interpolants),
we aim % would like
to strengthen it with data invariants
such that the proof establishes that the  path satisfies the safety property $\varphi$.
To do so, we generate a system of Horn clause constraints from the path in some
first-order theory admitting interpolation (e.g., linear arithmetic).
These Horn clauses carefully encode
the path's data manipulation along with the spatial interpolants,
which tell us heap shape at each location along the path.
The solution of this constraint system, which can be solved
using off-the-shelf first-order 
interpolant generation techniques (e.g.,~\cite{McMillan2011,Rybalchenko07}),
is a \emph{refinement} (strengthening) of the memory safety proof.
For example, we might transform an assertion 
$\ls(x,\nil)$ -- there is a linked list from $x$ to $\nil$ -- 
into the stronger formula $\ls(\lda{a.a > 0}, x, \nil)$ -- all elements of the list from $x$ to $\nil$
are greater than $0$.
We call the resulting annotations \emph{spatial interpolants modulo
theories} (or \emph{spatial($\theory$)} interpolants for short).
Note that our data refinements are \emph{not tied to a specific logical
theory} $\theory$, giving us a rather generic algorithm
and freedom to choose an appropriate theory to encode
a program's data.

Heap shapes are expressed using a fragment of separation logic with general
recursive predicates.  The (second-order) recursive predicates are
parameterized by data refinement predicates that at each unfolding are able to
constrain a finite history or window of the data stored in memory described by
the recursive predicate.  The recursive predicate definitions contribute to
the Horn constraints, and first-order interpolants are used to refine the data
refinement predicate parameters of recursive predicates.

We have implemented an instantiation of our generic technique 
in the \textsc{T2} safety and termination verification tool~\cite{t2},
and used it to prove correctness of a number of
programs, partly drawn from open source software,
requiring combined data and heap invariants.
Our results indicate the usability and promise
of our approach.

\paragraph{Contributions}
We summarize our contributions as follows:
\begin{compactitem}
\item A generic property-directed algorithm
for verifying and falsifying safety of programs with heap and data manipulation.

\item A precise and expressive separation logic analysis for computing memory safety
proofs of program paths using a novel technique we term \emph{spatial interpolation}.

\item A novel interpolation-based technique for strengthening
separation logic proofs with
data refinements.

\item An implementation and an evaluation of our technique for a fragment
of separation logic with linked lists enriched with linear arithmetic
refinements.
\end{compactitem}

\emph{The \textbf{appendix} contains an extended version
(A) a complete description of \alg, (B) proofs, 
(C) complete semantics and proof system of our program logic, and
(D) other extended clarifications.
}
%\paragraph{Organization}
%We start with an example
%illustrating the operations of our algorithm (Section~\ref{sec:ex}).
%In Section~\ref{sec:prelims}, we introduce
%definitions and notation required for the rest of the paper.
%In Sections~\ref{sec:spint} and~\ref{sec:snint},
%we formalize spatial interpolants modulo theories
%and describe an algorithm for computing them.
%In Section~\ref{sec:alg}, we describe
%how to construct a whole-program proof
%from proofs of individual paths.
%In Section~\ref{sec:impl},
%we describe our implementation and present
%our experimental results.
%Finally, in Section~\ref{sec:rel},
%we place our technique in the context of related work.
%

%The idea of property-directed verification is to compute an invariant that is,
%rather than the strongest possible, \emph{just strong enough} to prove that
%some desired property holds \cite{Henzinger2002,McMillan2006}.  The key
%benefit of property direction is that it enables scalable reasoning in rich
%program logics.  Property directed tools have proven to be much faster than
%abstract interpretation based techniques when the properties that one hopes to
%verify are simple and local to a part of the program.  \zak{It may very well
%  be that property directed tools can be faster than eager tools, but I
%  wouldn't say that it's been ``proven''.  And this is going to piss off half
%  the people reading the paper.  Also, we should be careful how we use the
%  word abstract interpretation -- there's no reason why an abstract
%  interpreter can't be property directed.}
%
%Separation logic \cite{Reynolds2002} based program verification tools have in
%recent years been shown to be effective at reasoning about heap-manipulating
%programs~\cite{Distefano2006,Yang2008}.  However, the question of making a
%property-driven tool that uses separation logic has remained open until now.
%{\bf WHY IS THAT? IS THERE A TECHNICAL HURDLE TO BE OVERCOME? WE SHOULD SAY
%  SO}.  \zak{Calling it an open problem implies that someone has (publicly)
%  asked for a solution, and we're providing it.  Is there something we can
%  cite for this?  I'm guessing that the only reason there haven't been
%  previous property-directed separation logic provers is that no one has tried
%  to make one.} In this paper, we present such an approach, based on {\bf
%  XXXXXXXXXXXXXXXX}.
%
%
%%% These techniques are all based on an ``eager'' strategy: they compute, at
%%% every program point, the strongest formula which holds for every state that
%%% can reach that point.  In contrast, many of the state-of-the-art tools for
%%% analyzing (heapless) \emph{integer} are based on ``lazy'' (or \emph{property
%%%   directed}) strategy: they compute, at every program point, a formula which
%%% is \emph{just strong enough} to prove that some desired property holds.
%
%%% Automated software verification techniques have seen remarkable success at
%%% proving interesting properties of programs in several application domains.
%%% Approaches based on \emph{separation logic} have been used to automatically
%%% establish sophisticated data structure invariants for heap-manipulating
%%% programs.
%
%%% For programs with integer variables, the \emph{lazy abstraction}
%%% paradigm is a powerful technique for proving numerical properties.  The domain
%%% of programs which require reasoning about the heap \emph{and} numerical
%%% properties is relatively less explored.  This paper presents \emph{spatial
%%%   interpolation}, a technique which combines separation logic and lazy
%%% abstraction to effectively reason about integer programs that manipulate the
%%% heap.
%
%{\bf BYRON SAYS: I DONT THINK THAT THIS IS THE PLACE TO TALK ABOUT THIS. JUST
%DESCRIB£E THE TECHNIQUE VIA AN EXMPLE IN THE NEXT SECTION. }
%\zak{What does ``this'' refer to?  The commented-out part or the italics part?
%  I think starting with an example is a good way to make everything concrete.}
%{\em
%Consider the following program, which allocates
%a list of random numbers and then computes the frequency of each number in
%the list:
%
%\begin{lstlisting}[language=C,caption=Frequency counting program]
%int freq[50];
%xs = null;
%while(*) {
%  a = rand() % 50;
%  xs = cons(a, xs);
%}
%
%while(xs != null) {
%  a = xs->data;
%  freq[a] = freq[a] + 1;
%  xs = xs->next;
%}
%\end{lstlisting}
%\label{lst:freq}
%
%The memory safety of this second loop in this program relies on the
%precondition that \texttt{xs} points to a null-terminated list.  This
%spatial property alone is not enough to prove safety: in order for the array
%access \texttt{freq[a]} to be safe, we must know that each element of the list
%pointed to by \texttt{xs} is a valid index into the array \texttt{freq}.  This
%is a combined heap/data property of the type addressed by this paper.
%
%A first step towards tackling heap/data problems is defining a
%program logic can be used to reason about the heap and integers
%simultaneously.  In this paper, we define a variation of separation logic that
%is suited to this purpose.  In our logic, we allow for the typical recursive
%predicates of separation logic (e.g., the \emph{list segment} predicate $\ls$)
%to be \emph{refined} by data predicates (drawn from some pure data theory, such as linear arithmetic).  For example, we can express the
%invariant required to prove memory safety of Listing~\ref{lst:freq} using the
%following refined list segment predicate:
%\[ \ls(0 \leq \nu < 50, \texttt{xs}, \nil) \]
%The interpretation of this formula is that \texttt{xs} points to a
%\nil-terminated list such each element $e$ of the list satisfies the
%property $0 \leq e < 50$.
%
%This logic is quite expressive, which often presents a barrier to tractable
%automated reasoning.  The main contribution of this paper is an algorithm
%which overcomes this barrier by taking advantage of property direction.  The
%algorithm takes as input a program $P$ with a designated error location.  The
%goal of the algorithm is either to prove that the error location is reachable,
%or to provide a path of program $P$ that demonstrates that either (1) the
%error location is reachable, or (2) the program is not memory safe.
%
%
%
%The algorithm, depicted in Figure~\ref{fig:arch}, operates similarly to
%McMillan's \textsc{Impact} algorithm.  First, we query the \emph{verifier} for
%a path to the error location that has not yet been shown to be infeasible.  We
%then symbolically execute $\pi$, which produces a sequence of symbolic heaps
%along the longest prefix $\pi'$ of $\pi$ that is memory safe.  If $\pi'$ is
%feasible, then we are done: $\pi'$ is a counterexample which proves that that
%the program is incorrect (either the error location is reachable or the
%program is not memory safe).  If $\pi'$ is infeasible, then we must decorate
%$\pi'$ with intermediate assertions to prove that it is infeasible.  This
%proceeds in two steps: (1) the \emph{heap prover} computes a separation logic
%proof of memory safety of $\pi'$, and (2) the \emph{data prover} computes
%data refinements for that memory safety proof which proves that $\pi'$ is
%infeasible.  Having proved that $\pi$ is a spurious counter-example, the
%algorithm proceeds to query the verifier for another program path, until all
%paths in the program are covered.
%}

